Concurrent Shuffle Differential Privacy Under Continual Observation

We introduce the concurrent shuffle model of differential privacy. In this model we have multiple concurrent shufflers permuting messages from different, possibly overlapping, batches of users. Similarly to the standard (single) shuffle model, the privacy requirement is that the concatenation of all shuffled messages should be differentially private. We study the private continual summation problem (a.k.a. the counter problem) and show that the concurrent shuffle model allows for significantly improved error compared to a standard (single) shuffle model. Specifically, we give a summation algorithm with error $\tilde{O}(n^{1/(2k+1)})$ with $k$ concurrent shufflers on a sequence of length $n$. Furthermore, we prove that this bound is tight for any $k$, even if the algorithm can choose the sizes of the batches adaptively. For $k=\log n$ shufflers, the resulting error is polylogarithmic, much better than $\tilde{\Theta}(n^{1/3})$ which we show is the smallest possible with a single shuffler. We use our online summation algorithm to get algorithms with improved regret bounds for the contextual linear bandit problem. In particular we get optimal $\tilde{O}(\sqrt{n})$ regret with $k= \tilde{\Omega}(\log n)$ concurrent shufflers.

==> nonsampling.tex <==
\section{No sampling}
The following algorithm works with probability 0.5, and should be boosted $\log{1/\delta}$ times to work with high probability $\geq 1-\delta$.

\begin{algorithm}[H]\label{alg:abc}
\SetAlgoLined
\textbf{Input:} $n$ data points $X$, thresholds $r>0$ and $c>1$, privacy parameter $\eps$, and maximal number of queries $m$.\\
\textbf{Initialize:} Let $H_{near}$ be an $(r,$\red{$\sqrt{c}$}$r,p_1,p_2)$-LSH hash family and $H_{far}$ be an $($\red{$\sqrt{c}$}$r,$\red{$c$}$r,p_1',p_2')$-LSH hash family\;
Let $\rho=\frac{\log p_1}{\log p_2}$, $k=\log_{1/p_2}(n)$ (i.e., $p_2^k=1/n$), $L=n^\rho \log n \cdot 16\log (10n)$, $\rho'=\frac{\log {p_1'}}{\log {p_2'}}$, $k'=\log_{1/{p_2'}}(n)$ (i.e., ${p_2'}^k=1/n$), $L'=n^{\rho'} \log n \cdot \frac{16\log (10n)}{\eps}$ and $Y=10L+1$\;
Let the hash functions $\{h^j_{near}\}_{j=1}^{L}$ sampled iid and uniformly from $H_{near}^k$ and the hash functions $\{h^j_{far}\}_{j=1}^{L'}$ sampled iid and uniformly from $H_{far}^k$\;
Create the data structures $L$ and $L'$ mapping each k-concatenated hash to the set of points which map to it in the near and far structures respectively\;
 \For{query $q_t$ for $t\gets1,2,\ldots m$}{
    % \red{The following lines until "otherwise" might be redundant\;}
    % Sample $\sqrt{n}$ data points $x_1,\ldots, x_{\sqrt{n}}$ uniformly with replacements from $X$\;
    % Compute the distances $d(q_t,x_1),\ldots, d(q_t,x_{\sqrt{n}})$\;
    % If any point is of distance at most $cr$ to $q_t$, return it and exit\;
    % Otherwise, fetch 
    Fetch the set $A$ of the first $Y$ points from the near LSH structure buckets $\{h^{j}_{near}(q_t)\}_{j=1}^{L}$ (by iterating over them, and breaking once we see sufficiently many points)\;
    Simulate \textbf{\textit{Report Noisy Max}} (tuned for $(\eps/m)$-DP) over the set of points $a\in A$ for the far LSH counting function $count(a)=|\{j:h^{j}_{far}(q_t)=h_j(a)\}|$, and stop once we find the first point\;
    \red{TODO: This is probably not DP however, since the set for ranking is different from the set for retrieval, and it is sensitive to the set for retrieval.}
 }
 \caption{Adversarially Robust LSH}
\end{algorithm}

\begin{theorem}[robustness]
    The algorithm above is $\eps$-DP with respect to the hash functions.
    \red{TODO: connect DP to the notion of robustness.}
\end{theorem}
\begin{proof}
\red{How do I relate the flip number and $\lambda$ to this problem?}
This is clear since the output of the mechanism is $(\eps/m)$-DP in every iteration, so the total privacy loss over the $m$ iterations is $\eps$. \red{Make sure that because I break after a few points, I'm not to sensitive to the first hash. This is currently the problem.}
Question: what must $\eps$ be for it to be robust?

\end{proof}

\begin{theorem}[complexity]
    The data structure above takes $O\left(n^{1+\rho}\log^2n+\frac{n^{1+\rho'}\log^2n}{\eps}\right)$ memory and runtime to create, and for each query runs in $O\left(\frac{n^{\rho+\rho'}\log^4n}{\eps}\right)$ time.
\end{theorem}
\begin{proof}
Note that we go over at most $L$ hash buckets, and we break once we scan $Y$ points. Hence, the first part of the algorithm takes $O(L+Y)$ runtime. The application of Report Noisy Max takes time which is linear in the domain size $O(Y)$ and each computed match count takes $O(L')$ (go over hashes and count collisions), so this takes $O(L'Y)$, and the total runtime per query is $O(L+L'Y)=O(L+L'\cdot 10L)=O(L'\cdot L)=O\left(\frac{n^{\rho+\rho'}\log^4n}{\eps}\right)$, where the last one follows by the definition of $L$. If we include the hash computation time $O(d)$, we get an additional multiplicative $O(d)$ factor.

For the memory and time to create the data structure, we create $L$ near LSH structures, and $L'$ for ones, and compute hashes of the $n$ points to create each, so it requires $O(n(L+L'))=O\left(n^{1+\rho}\log^2n+\frac{n^{1+\rho'}\log^2n}{\eps}\right)$ memory and runtime.
\end{proof}

\begin{theorem}[accuracy/correctness]
    The algorithm finds a $cr$-nn with high probability.
\end{theorem}
\begin{proof}
    In order to prove that the algorithm finds an $(r,cr)$-ANN with high probability, we must show that if there exists an $r$-neighbor to the query, then with high probability we find a $cr$-neighbor to the query.
    
    Indeed, assume that the point $z_r$ is of distance at most $r$ to $q_t$. 
    % Note that any point that is returned in the $\sqrt{n}$ sampling phase is of distance at most $cr$ to $q_t$ and therefore an approximate near neighbor as required.
    
    % We therefore consider the case that no such point was found, and we continue to the second part of the algorithm.
    Recall that the algorithm selects the first $Y$ points among the set $S$ of all points $x$ such that exists $i\in [L]$ which match the query with a hash from the near family $h^i_{near}(x)=h^i_{near}(query)$ by going over the $L$ hash tables, and then selects the approximate one who matched the largest number of hashes for the far hash family $h^j_{far}(x)=h^j_{far}(query)$.
    
    We define 5 events which combined together will guarantee that we return a $cr$-nn.
    \begin{enumerate}
        \item $E_1$ the point $z_{r}$ (of distance at most $r$ to query), matches at least one near hash with the query.
        \item $E_2=$ the number of non-$\sqrt{c}r$-nn gathered throughout the $L$ near LSH buckets is at most $10L$.
        \item $E_3=$ Report Noisy Max on the gathered data points returns a point which matches at least the opt minus $\frac{4\log (10n)}{\eps}$ far hashes with the query.
        \item $E_4=$ the number of far hash matches of $z_{\sqrt{c}r}$ with the query is at least $\frac{L{p_1'}^k}{2}$.
        \item $E_5=$ there is no non-$cr$-nn which matches at least $2+\sqrt{6 \log (20n)}$ far hashes with the query. 
    \end{enumerate}
    
    First, $E_2$ implies that out of the possible $10L+1$ retrieved items, at most $10L$ of them are non-$\sqrt{c}r$-nn points. By $E_1$, the point $z_{r}$ which is some $r$-nn matches some hash, so the last available spot can be either taken by $z_{r}$ or by some other point of distance at most $\sqrt{c}r$ to the query which matched a hash before $z_{r}$ (it cannot be taken by a farther point since we bounded their number by $10L$), so we do indeed fetch some point $z_{\sqrt{c}r}$ of distance at most $\sqrt{c}r$ to the query.
    
    Last, $E_4$ shows that the optimal point has at least $\frac{L{p_1'}^k}{2}$ far LSH matches (since specifically $z_{\sqrt{c}r}$ was retrieved in the first step, and it has such a quality), and therefore by $E_3$, the algorithm returns a point with at least the following number of hash matches with the query:
    \begin{align*}
        \frac{L{p_1'}^k}{2}-\frac{4\log (10n)}{\eps}\geq \frac{8\log (10n)}{\eps}-\frac{4\log (10n)}{\eps}\geq \frac{4\log (10n)}{\eps}\geq 2+\sqrt{6 \log (20n)},
    \end{align*}
    where the first step follows since $L{p_1'}^k>\frac{16\log (10n)}{\eps}$ which follows since ${p_1'}^k=n^{-\rho}$ and by the definition of $L$, and the last step follows since $4\log (10n)\geq 2+\sqrt{6 \log (20n)}$ for any $n>1$ and since $\eps<1$.
    
    Thus, by $E_5$, the returned point must be a $cr$-nn, as required.
    
    We now bound the probability that each of the events occurs.
    \begin{enumerate}
        \item \textbf{$E_1$:} 
        % On the other hand, the good event $B$ in which the $L$ buckets to include the $cr$-distant point [i.e., we recover the point], 
        Notice that since the $L$ buckets are independent, the probability that we retrieve $z_r$ in at least one of them is at least $1-(1-p_1^k)^L$. However,
        % Therefore, $P(retrieved-z-in-some-hash)=P(A\wedge B)\geq 1-P(\bar{A})-P(\bar{B})\geq 1-\frac{1}{10}-(1-p_1^k)^L$. 
        \begin{align*}
            1-(1-p_1^k)^L&=1-(1-p_2^{\rho k})^L=1-(1-p_2^{\rho k})^L=1-(1-(1/n)^{\rho})^L\\
            &\geq 1-e^{-(1/n)^\rho\cdot L}=1-e^{-\log n}=1-\frac{1}{n}\geq \frac{9}{10},
        \end{align*}
        where the first step follows by the definition of $\rho$ and the sixth step follows by the definition of $L$ and since $16 \log (10n)>1$ since $n>1$, and the last step follows since we assume $n>10$.
        
        \item \textbf{$E_2$:} for each hash table $j\in [L]$, consider the random variable of the number of non-$\sqrt{c}r$-nn collisions. Since there are at most $n$ bad points, and each one of them collides with probability at most $p_2^k$, by the linearity of expectation each hash table we get expected $np_2^k=1$ (by the definition of $k$) bad points, so expected total $L$ bad points over all the buckets. Therefore, by Markov inequality, the number of bad points throughout the $L$ buckets is at most $10L$ with probability at least $\frac{9}{10}$. \\
    
        \item \textbf{$E_3$:} Recall that the algorithm returns a private estimate of the point which agrees with the query on the most far LSH hash values.
        Specifically, the quality of each retrieved point is the number of far LSH $k$-hashes it matches with the query, and we report the noisy max for this quality function, protecting each hash function.   

    
    
    
    
    
    
    
%     Since there are at most $\sqrt{n}$ near points, we don't expect to retrieve more than $\sqrt{n}\cdot L$ positive points in total. So in total we expect to get at most $Y=nL\cdot p_2^k+\sqrt{n}L$ points.\footnote{Note that $L=n^\rho$, so for the algorithm to be sublinear, we must have $\rho<1/2$ or alternatively to change the $\sqrt{n}$ used in this algorithm with another exponent that depends on rho.}
% Now, we take the element $s \in S$ which matches the query in the largest number of hashes among $h_1,...,h_L$.  

% We can't do it directly since it isn't robust and releases info about the hashes, but we can release the DP value wrt the hashes. Specifically, we report noisy max for the query which matches most hashes.

% Note that the accuracy loss (the additive diff from the optimal to what it returns) of report noisy max is order of $\frac{sensitivity\cdot \ln(\#outputs)}{\eps}$. Here, the sensitivity is 1, since the value of each counter can change by at most 1 when we change the hash function $h_i$. Therefore, the additive diff is order of $\frac{\ln(\#gathered-points)}{\eps}\leq \frac{\ln(\#gathered-points)}{\eps}$. 
% More formally,
The following proposition is well-known about the report-noisy-max mechanism:
\begin{proposition}[Proposition 15 in \href{https://eprint.iacr.org/2016/820.pdf}{https://eprint.iacr.org/2016/820.pdf}]
For any $\beta$, w.p. $P\left(quality(ReportNoisyMax(D))\geq opt-\frac{4(\log{(\#outputs)}+\log \frac{1}{\beta})}{\eps}\right)\geq 1-\beta$.
\end{proposition}
Applied to our algorithm, where we have at most $Y\leq n$ outputs, and taking $\beta=\frac{1}{10}$ this means that 
\begin{equation*}
    P\left(E_3\right)=P\left(quality(ReportNoisyMax(D))\geq opt-\frac{4\log (10n)}{\eps}\right)\geq \frac{9}{10}.
\end{equation*}

\item \textbf{$E_4$:} From the perspective of a single data point, the number of collisions is a binomial distribution (each uniform hash from the family has the same collision probability). Hence, we use a specific version of Chernoff bounds which arises from Theorem E.1 in Cheu et al.~\href{https://arxiv.org/abs/1808.01394}{https://arxiv.org/abs/1808.01394}.
\begin{lemma}\label{lma:chernoff}
For any binomial distribution $Bin(n,p)$ and $\delta>0$ it holds that $$P\left(\abs{B-np}\geq \sqrt{3np\log \frac{2}{\delta}}\right)<\delta.$$
\end{lemma}

For $z_{\sqrt{c}r}$, by Lemma~\ref{lma:chernoff}, since its far LSH hash collision probability is $p\geq {p_1'}^k$, then
$$ P\left(\#matches-of-z\geq L'p- \sqrt{3L'p\log (20)}\right) \geq \frac{9}{10}.$$
Note that since $L'p\geq L'{p_1'}^k\geq 12\log (20)$ (MAKE SURE), then $\frac{L'p}{2}\leq L'p-\sqrt{3L'p\log (20)}$
and therefore:
\begin{equation*}
    P\left(\#matches-of-z\geq \frac{L'{p_1'}^k}{2}\right) \geq \frac{9}{10}.
\end{equation*}

\item \textbf{$E_5$:} 
For any non-$cr$-nn $u$, assuming its collision probability is $p\leq {p_2'}^k$, we get that
\begin{align*}
    P\left(\#matches-of-u\geq 1+\sqrt{3\log \frac{2}{\delta}}\right)&\leq  
    P\left(\#matches-of-u\geq Lp+\sqrt{3Lp\log \frac{2}{\delta}}\right)<\delta,
\end{align*}
where the first step follows since $L'p\leq L'{p_2'}^k\leq n{p_2'}^k= 1$ (MAKE SURE $L'\leq n$. This must be since otherwise we are superlinear query time), and the second step follows by Lemma~\ref{lma:chernoff}.
Therefore, by a union bound over all the ($n$ at most) non-$cr$-nn points $u$ simultaneously, and taking $\delta=\frac{1}{10}$, we get that:
\begin{equation*}\label{eq:nonneighbors-low}
P\left(E_5\right)=P\left(\exists non-cr-nn-with-\#matches\geq 2+\sqrt{6 \log (20n)}\right)<\frac{1}{10}.
\end{equation*}
\end{enumerate}
We conclude that:
\begin{align*}
    P(returns-cr-nn)&\geq P(E_1\cap E_2\cap E_3\cap E_4\cap E_5)\\
    &= 1- P(E_1\cup E_2\cup E_3\cup E_4\cup E_5) \geq 1- \sum_{i=1}^{5} P(E_i)\\
    &=1-\frac{5}{10}=\frac{1}{2}, 
\end{align*}
i.e., the algorithm works with constant probability.
% To conclude that wp $\geq 0.7$, there is point with quality at least $\frac{Lp_1^k}{2}$, no non-$cr$-nn passes quality $2+\sqrt{6 \log (20n)}$, and the mechanism returns a point with quality at least the optimum (which by just above is least $\frac{Lp_1^k}{2}$) minus $\frac{4\log (10n)}{\eps}$. Thus, proving $\frac{Lp_1^k}{2}-(2+\sqrt{6 \log (20n)})\geq \frac{4\log (10n)}{\eps}$ will yield that we return a $cr$-nn with probability $\geq 0.7$. 

% Note that if we ensure that the additive diff $\frac{\ln(n)}{\eps}$ is smaller than the diff that should be for separating $r$-near points with farther than cr near points, we finish.
% Indeed, the $r$-nn point $z$ matches each hash with probability $p_1^k$, so it is expected to match $Lp_1^k$ hashes [and is pretty concentrated by chernoff, with stdev $\sqrt{expectation}=\sqrt{L}p_1^{k/2}$]. Each point of distance at least $cr$ is expected to match $Lp_2^k$ hashes [and is pretty concentrated by chernoff, with stdev $\sqrt{expectation}=\sqrt{L}p_2^{k/2}$].
% Therefore, for the separation, over all the points we need that:
% $$Lp_1^k-\sqrt{Lp_1^k}-Lp_2^k+\sqrt{Lp_2^k}   >   \frac{\ln(Y)}{\eps}.$$

% Indeed, 
% \begin{align*}
%     Lp_1^k-\sqrt{Lp_1^k}-Lp_2^k+\sqrt{Lp_2^k}&> Lp_1^k-\sqrt{Lp_1^k}-Lp_2^k\\
%     &\geq \frac{1}{2}Lp_1^k-Lp_2^k\\
%     &\geq \frac{1}{2}Lp_1^k-np_2^k\\
%     &= \frac{1}{2}Lp_1^k-1\\
%     &\geq \frac{1}{2}Lp_1^k-\frac{\ln (Y)}{\eps}\\
%     &\geq \frac{2\ln (Y)}{\eps}-\frac{\ln (Y)}{\eps}=\frac{\ln (Y)}{\eps}
% \end{align*}
% where the second step follows since $Lp_1^k\geq 4$ (\red{TODO: make sure this happens by selecting $L$ accordingly}) and for $x\geq 4$ it holds that $\sqrt{x}\leq x/2$, the third step follows since $L\leq n$ (\red{TODO: make sure this happens by selecting $L$ accordingly. This should happen since otherwise $L>n$ and we are no longer a sublinear algorithm}), the fourth step follows by the definition of $k$, the fifth step follows since $Y>2$ and $\eps<1$, and the last step follows since $Lp_1^k>\frac{4\ln (Y)}{\eps}$ by the definition of $L=n^\rho\cdot \frac{4\ln(Y)}{\eps}$ (note that in regular LSH we have that $L>n^\rho$ gives $Lp_1^k>1$, so we get the additional $\frac{1}{\eps}$ term).

% but it suffices to show that:
% $$Lp_1^k-Lp_2^k-\sqrt{Lp_1^k}   >   \frac{\ln(Y)}{\eps}.$$

% Since $L<n$ (otherwise we go over at least $n$ hashes and the algorithm is no longer sublinear) then this means that $Lp_2^k<n\cdot \frac{1}{n}<1$, where since $Lp_1^k$ must be anyways larger than $\frac{\ln(Y)}{\eps}$, makes $Lp_2^k$ negligible, and it satisfies to select params such that roughly:
% $$Lp_1^k-\sqrt{Lp_1^k}  >   \frac{\ln(Y)}{\eps}.$$
% Since anyways $\frac{\ln(Y)}{\eps}>1$, then we need $Lp_1^k>1$, and therefore the sqrt of $Lp_1^k$ is at most half of it, and therefore up to a 2-constant we need:
% $$Lp_1^k  >   \frac{\ln(Y)}{\eps}.$$












%     Otherwise, whp we are in the case of less than $\sqrt{n}$ points of distance at most $cr$ to the query. We gather the set $S$ of all the points $x$ such that exists $i\in [L]$ for which $h_i(x)=h_i(query)$ by going over the $L$ hash tables.
    
%     Since for each i we have a mistaken collision wp $<q$, then the total expected number of false positive collisions throughout the $L$ tables is at most $nL\cdot p_2^k$. We expect to include the $cr$-distant point [i.e., succeed] with probability at least $1-(1-p_1^k)^L$. Since there are at most $\sqrt{n}$ near points, we don't expect to retrieve more than $\sqrt{n}\cdot L$ positive points in total. So in total we expect to get at most $Y=nL\cdot p_2^k+\sqrt{n}L$ points.\footnote{Note that $L=n^\rho$, so for the algorithm to be sublinear, we must have $\rho<1/2$ or alternatively to change the $\sqrt{n}$ used in this algorithm with another exponent that depends on rho.}
% Now, we take the element $s \in S$ which matches the query in the largest number of hashes among $h_1,...,h_L$.  

% We can't do it directly since it isn't robust and releases info about the hashes, but we can release the DP value wrt the hashes. Specifically, we report noisy max for the query which matches most hashes.

% Note that the accuracy loss (the additive diff from the optimal to what it returns) of report noisy max is order of $\frac{sensitivity\cdot \ln(\#outputs)}{\eps}$. Here, the sensitivity is 1, since the value of each counter can change by at most 1 when we change the hash function $h_i$. Therefore, the additive diff is order of $\frac{\ln(Y)}{\eps}$. 

% Note that if we ensure that the additive diff $\frac{\ln(Y)}{\eps}$ is smaller than the diff that should be for separating $r$-near points with farther than cr near points, we finish.
% Indeed, if there is a point of distance at most $r$, it matches each hash with probability $p_1^k$, so it is expected to match $Lp_1^k$ hashes [and is pretty concentrated by chernoff, with stdev $\sqrt{expectation}=\sqrt{L}p_1^{k/2}$]. For points of distance at least $cr$, it's expected to match $Lp_2^k$ hashes [and is pretty concentrated by chernoff, with stdev $\sqrt{expectation}=\sqrt{L}p_2^{k/2}$].
% Therefore, for the separation we need that:
% $$Lp_1^k-\sqrt{Lp_1^k}-Lp_2^k+\sqrt{Lp_2^k}   >   \frac{\ln(Y)}{\eps},$$
% Which since $\sqrt{Lp_1^k}>\sqrt{Lp_2^k}$ can be roughly written as:
% $$Lp_1^k-Lp_2^k-2\sqrt{Lp_1^k}   >   \frac{\ln(Y)}{\eps}.$$
% Note that in the regular LSH params where $p_2^k=1/n$ (i.e., $k=\log_{1/p_2}(n)$), then the dominant term in $Y$ is $\sqrt{n}L$, so $\ln{Y}$ is roughly $\ln(n)+\ln(L)$. Since $L<n$ then this means that $Lp_2^k<n\cdot \frac{1}{n}<1$, where since $Lp_1^k$ must be anyways larger than $\frac{\ln(Y)}{\eps}$, makes $Lp_2^k$ negligible, and it satisfies to select params such that roughly:
% $$Lp_1^k-2\sqrt{Lp_1^k}  >   \frac{\ln(Y)}{\eps}.$$
% Since anyways $\frac{\ln(Y)}{\eps}>1$, then we need $Lp_1^k>1$, and therefore the sqrt of $Lp_1^k$ is at most half of it, and therefore up to a 2-constant we need:
% $$Lp_1^k  >   \frac{\ln(Y)}{\eps}.$$
% In regular LSH we roughly have the requirement $Lp_1^k>1$ which amounts to $L>n^\rho$, but here we have in RHS $\frac{\ln(Y)}{\eps}$, so we get $L=n^\rho\cdot \frac{\ln(Y)}{\eps}$.
% Note that in this definition of L, we have Y which depends on L itself. So we want to bound Y to understand how large L must be. 
% Since Y is roughly ???, by L's definition above, $\ln{L}$ is roughly $\rho\cdot \ln{n}=\ln{n}$, so y is roughly $
% \ln{n}$, and we get that roughly $L=n^\rho\cdot \frac{\ln(Y)}{\eps}$.
% Therefore in total we expect to get at most $Y=nL\cdot p_2^k+\sqrt{n}L=L+\sqrt{n}L\approx \sqrt{n}L=n^{\rho+0.5}
% \cdot \frac{\ln(Y)}{\eps}$ points.
% This means that $\rho$ must be smaller than 0.5 for it to be sublinear.
% Data-dependent LSH is $\rho=\frac{1}{2c^2-1}$ and for hamming it is $\rho=\frac{1}{2c-1}$. The data-independent LSH is something like $\rho=1/c$.
% Question: what must $\eps$ be for it to be robust?

\red{TODO: boost the probablity to $1-\delta$, we perform the process on $\log \frac{1}{\delta}$ independent such structures. Adjust all proofs accordingly.}
\end{proof}

==> obsolete.tex <==
\subsection{Taking a DP algorithm with expected runtime E which works with const prob and making it DP with worst case runtime E' which works WHP.}

\begin{algorithm}[H]\label{alg:expectedToWHP}
\SetAlgoLined
\textbf{Input:} $(\eps,\delta)$-DP alg $M$ with expected runtime $\leq E$ for every input.\\
 \For{$i=1,\ldots,\log (1/\delta)$}{
    Run $M$ for $10E$ steps, and if it returned an answer, return it\;
 }
 Fail\;
 \caption{Boosting DP}
\end{algorithm}

\begin{theorem}
    Algorithm~\ref{alg:expectedToWHP} is $\left(\eps\log (1/\delta), \delta\log (1/\delta)\right)$-DP with worst case runtime $O\left(E\log (1/\delta)\right)$, and returns a result with the same output distribution as $M$ on the input, with probability $\geq 1-\delta$.
\end{theorem}
\begin{proof}
    By composition rules, running the algorithm $\log (1/\delta)$ times means the algorithm is $\left(\eps\log (1/\delta), \delta\log (1/\delta)\right)$-DP.
    
    Since we run $\log (1/\delta)$ times an algorithm for $10E$ steps, the total runtime is at most $10E\log (1/\delta)=O\left(E\log (1/\delta)\right)$.
    
    Since the expected runtime of the algorithm on the input is $\leq E$, by Markov's inequality, $P(runtime\leq 10E)\geq 9/10$, and therefore the probability that at least one iteration succeeds is $\geq 1-\frac{1}{10^{\log (1/\delta)}}\geq 1-\delta$, and we return its answer.
    
    \red{Why is the output distribution the same? What if there is a correlation between the output and the runtime taken to give the output? If thereis no such correlation, it should work.}
\end{proof}



Assume that the $m$'th batch is with the users $2^{m-1}+1$ until $2^m$.
\section{Proof}
For the rest of the proof, we condition on assumption A.1, which holds wp $\geq 1-\alpha$. 

Define $G_m=\sum_{t=1}^{2^m}\phi(c_t,a_t)\phi(c_t,a_t)^T$ and $V_m=G_m+H_m$ where $H_m=\lambda I_d+\sum_{i=1}^{m}N_m$. Consider also the error $h_m=\sum_{i=1}^{m}n_m$.

\textbf{$\hat{\theta}_m$ is near $\theta^*$ with the confidence radii $\beta_m$ for all batches $m=1,\ldots,\log T$:}

\begin{align}
    \theta^*-\hat{\theta}_m &= \theta^*-V_m^{-1}u_m\\
    &=\theta^*-\left(G_m+\lambda I_d+\sum_{i=1}^{m}N_m\right)^{-1}
    \left(\sum_{t=1}^{2^m}\phi(c_t,a_t)y_t+\sum_{i=1}^{m}n_m\right)\\
    &=\theta^*-\left(G_m+H_m\right)^{-1}
    \left(\sum_{t=1}^{2^m}\phi(c_t,a_t)y_t+h_m\right)\\
    &=V_m^{-1}\left(H_m\theta^*-\sum_{t=1}^{2^m}\phi(c_t,a_t)\eta_t-h_m\right)
    ,
\end{align}
where the fourth step follows since $y_t=\ip{\phi(c_t,a_t)}{\theta^*}+\eta_t$ and from elementary algebra.

Thus multiplying both sides by $V_m^{1/2}$ gives 

\begin{align}
    \norm{\theta^*-\hat{\theta}_m}_{V_m} &\leq  \norm{H_m\theta^*}_{V_m^{-1}}+\norm{\sum_{t=1}^{2^m}\phi(c_t,a_t)\eta_t}_{V_m^{-1}}+\norm{h_m}_{V_m^{-1}}\\
    &\leq \norm{\theta^*}_{H_m}+\norm{\sum_{t=1}^{2^m}\phi(c_t,a_t)\eta_t}_{(G_m+\lambda_{min}I)^{-1}}+\norm{h_m}_{H_m^{-1}}
    ,
\end{align}
where the second step follows since $V_m\geq H_m,~V_m\geq G_m+\lambda_{min}I$ by assumption A1. The first and third terms are bounded by using A1 and the fact that $\theta^*$ is bounded. We now bound the middle term.


This continues as the original proof, but $M=\log T$ instead of $M=T/B$ and $t_m=2^m$ instead of $t_m=B\cdot m$.

We define $\Gamma_i(\cdot , \cdot):=\beta_{\floor{T}_2}\cdot \norm{\phi(c_t,a_t)}_{\hat{V_i}^{-1}}$, where $\hat{V_i}=\sum_{t=1}^{i}\phi(c_t,a_t)\phi(c_t,a_t)^T +\lambda_{min}I_d$.
As in page 19 on top, defining $\floor{t}_2$ as the largest power of 2 which is at most $t$ (i.e., round downwards to closest power of 2) we get 
\begin{equation}
    R(T)\leq \sum_{t=1}^{T} \min \left(2\Gamma_{\floor{t}_2}(c_t,a_t), 1\right),
\end{equation}
where the second part of the minimum is since the reward is bounded by 1 by the assumptions about the problem.
Define $\psi = \{t\in [T] \mid \Gamma_{\floor{t}_2}(c_t,a_t)/\Gamma_{t-1}(c_t,a_t)>2\}$, then $|\psi|=\sum_{i=1}^{\log T}\sum_{t=2^i+1}^{2^{i+1}} 1_{\Gamma_{2^i}(c_t,a_t)/\Gamma_{t-1}(c_t,a_t)>2}\leq \sum_{i=1}^{\log T}\sum_{t=2^i+1}^{2^{i+1}} \left(\log  det(\hat{V}_{t-1})-\log  det(\hat{V}_{2^i})\right)$.
Let $\hat{\psi}=$

\section{Lower bound proving the exponential batch effort fails (for the adversarial case in contextual bandits)}
From https://arxiv.org/pdf/2004.06321.pdf\\
\includegraphics[width=\textwidth]{Screen Shot 2022-03-17 at 12.02.18.png}
Therefore, we can't do with exponentially growing batches since then the number of batches is $\log T$, and the lower bound has the component $\frac{T}{\sqrt{M}}=\frac{T}{\sqrt{\log T}}$ and specifically we can't recover $\sqrt{T}$ runtime.

For the non-adversarial case they do have hope:\\
\includegraphics[width=\textwidth]{Screen Shot 2022-03-17 at 12.25.17.png}
However, for linear bandits with stochastic contexts, $\sqrt{T}/\eps$ regret can be achieved even in the local model (this is optimal for the local model, but maybe the dependency on $\eps$ can be improved for the shuffle model to match the $\sqrt{T}/\sqrt{\eps}$ from JDP in the centralized model [it can even maybe pass this, since this bound is for adversarial contexts]).
Therefore in Zhou's paper they solve the problem when there are adversarial context and therefore cant get the $\sqrt{T}$ type regret, but using constant size batches of $B = O(T^{3/5})$, they get regret $O(T^{3/5}/\sqrt{\eps})$.









\begin{theorem}
For every $\eps\in [0,1/2]$ and $\delta \in [0,0.01]$, and any $(\eps,\delta)$-SDP $n$-user algorithm $M$ under continual observation with consecutive predetermined batches $B_1,\ldots,B_m$, there is an input data set $x \in X^n$ on which $M$ has error $\alpha = \Omega(\max_i\abs{B_i})$, and an input data set $y \in X^n$ on which $M$ has error $\alpha = \Omega(\sqrt{m})$, with constant \red{high?} probability.
\end{theorem}
\begin{proof}
Recall that as in the MAB paper, batches came one after the other. On one hand, observe that within the batch $B_i$, the error in the count right before the last user can be $\abs{B_i}-1$, since there is no update sent to the server within the batch, and the batch could be all 0's or all 1's. Therefore, there exists an input for which the error is $\Omega(\max_i\abs{B_i})$ with constant probability.

Consider a uniformly random input dataset $D = (d_1,\ldots, d_n)$ from the distribution where each $d_i$ is constant 0, except those which are the last of their batch which are sampled from $Ber(1/2)$, i.e., $\forall t\in[1,\ldots,m],~d_{\sum_{j=1}^{t}\abs{B_j}}\sim Ber(1/2)$, let $R = (R_1, \ldots, R_{m})$ denote the randomness of the $m$ batches, each $R_i$ which is in fact the randomness $\{R_i^j\}_{j=1}^{m}$ of the users of the batch $B_i$ together with the shuffle randomness, and let $T = T(D, R)$ be the random variable denoting the transcript of the protocol as sent to the server (the shuffled encoded bits throughout all the batches). Let $t \in Supp(T)$ be any value of $T$. We
claim that conditioned on $T = t$:
\begin{enumerate}
    \item The $m$ random variables of the sums of the batches $\{X_j\}_{j=1}^{m}$ where $X_j=\sum_{i\in B_j}d_i$
are independent.
    \item Each $X_i\in \{0,1\}$ and $Pr[X_i = 1] \in (1/4,3/4)$.
\end{enumerate}
Item 1 is a general fact about interactive protocols - if the parties’ inputs start independent,
they remain independent conditioned on the transcript - and can be proven by induction on the
number of rounds of the protocol. For item 2, observe that by the definition of $\{d_i\}_{i=1}^{n}$, all but at most one in each batch are 0, so the sum $X_i$ of each batch $i$ must be either 0 or 1. Using differential privacy and Bayes’ Rule, for any batch $i$ and its last user $i^*$,
\begin{align}
    \frac{Pr[X_i=1 \mid T=t]}{Pr[X_i=0 \mid T=t]}&=\frac{Pr[d_{i^*}=1 \mid T=t]}{Pr[d_{i^*}=0 \mid T=t]} = \frac{Pr[T=t\mid d_{i^*}=1]\cdot Pr[d_{i^*}=1]/Pr[T=t]}{Pr[ T=t\mid d_{i^*}=0]\cdot Pr[d_{i^*}=0]/Pr[T=t]} \\
    &= \frac{Pr[T=t\mid d_{i^*}=1]\cdot 1/2}{Pr[ T=t\mid d_{i^*}=0]\cdot 1/2} = \frac{Pr[T=t\mid d_{i^*}=1]}{Pr[ T=t\mid d_{i^*}=0]}.
\end{align}

Observe that $d_{i^*}$ only affects the portion of the transcript $T$ of the batch $i$,\footnote{Since each new user has its predetermined batch and batch size, and their part of the communication is only affected by this, and is not a function of the history. Note that in dynamic batches however, the batch size and hence the communication is dependent of the history and specifically a previous $X_i$.} and shuffle differential privacy means the transcript within the batch is differentially private with respect to bit $d_{i^*}$ of the user $i^*$, so we get that $Pr[T=t\mid d_{i^*}=1]\leq e^\eps\cdot Pr[T=t\mid d_{i^*}=0]+\delta$ and $Pr[T=t\mid d_{i^*}=0]\leq e^\eps\cdot Pr[T=t\mid d_{i^*}=1]+\delta$. Combined with the equation above, this implies that 
$Pr[X_i=1 \mid T=t]\in \left[\frac{1-\delta}{e^\eps+1},\frac{e^\eps+\delta}{e^\eps+1}\right]\subseteq (1/4,3/4)$,
since $\eps\in [0,1/2]$ and $\delta \in [0,0.01]$.


Consequently, conditioned on $T = t$, $\sum_i X_i$ is the sum of $m$ independent random variables with bias in $(1/4,3/4)$ and specifically standard deviation at least $\sqrt{3}/4> 1/4$, and therefore has standard deviation at least $\sqrt{m}/4$. 

% In particular, the standard deviation of $\sum_i X_i$ is $\Omega(\sqrt{m})$, and by anti-concentration bounds, with high probability we will have
% $\abs{\sum_i X_i-output(t)}=\Omega(\sqrt{m})$,
% where $output(\cdot)$ is the output function of the protocol. Since the protocol has error $\Omega(\sqrt{m})$ on a random dataset with high probability, there is some fixed dataset on which it has error $\Omega(\sqrt{m})$ with high probability.

Bun et al.~\cite{bun2019heavy} establish the following anti-concentration bound:\\
``There exists constants $a,b,c>0$ s.t.\ the following holds. Let $X$ be a sum of independent random variables, each attaining values in $[0,1]$, and let $\sigma=\sqrt{Var[X]}\geq 200$. Then for all $a\geq \beta\geq2^{-b\sigma^2}$ and every interval $I\in \reals$ of length $\abs{I}\leq c\cdot \sqrt{\sigma^2\cdot \log (\frac{a}{\beta})}$ we have $Pr[X\notin I]\geq \beta$.''

Applying the above to the random variables $X_i\mid T=t$, we get that there are constants $a,b,c>0$ s.t.\ for all $a\geq \beta\geq2^{-bm/16}$ and every interval $I\in \reals$ of length $\abs{I}\leq c\cdot \sqrt{bm/16\cdot \log (\frac{a}{\beta})}$ we have $Pr[\sum_i X_i\notin I \mid T=t]\geq \beta$.
Specifically, given $T=t$, and defining $output(\cdot)$ as the output function of the protocol given the transcript, for the interval $I(t)=output(t) \pm c/2\cdot \sqrt{bm/16\cdot \log (\frac{a}{\beta})}$ it holds that $Pr\left[\abs{\sum_i X_i-output(t)}> c/2\cdot \sqrt{bm/16\cdot \log (\frac{a}{\beta})}\right]\geq \beta$. That means that with probability at least $\beta$ the protocol has error at least $\Omega(\sqrt{m})$ when estimating the sum of bits in the random dataset $D$. Hence, there must exist a fixed database on which it has error $\Omega(\sqrt{m})$ with probability greater than $\beta$.
\end{proof}
Therefore, the worst case error cannot be better than $\Omega(\max_i\abs{B_i},m))$, for which if there is batch of size at least $n^{1/3}$ then the error is at least $n^{1/3}$ and otherwise there are at least $m\geq n^{2/3}$ batches, and once again we get error at least $\Omega(\sqrt{n^{2/3}})=\Omega(n^{1/3})$. Therefore, in any case, for any predetermined static batch sizes, the worst case error is at least $\Omega(n^{1/3})$.

TODO: I can also extend to static batches trivially, and then to dynamic batches, and also to each user is in several batches.
For dynamic: if we know there are m batches apriori, and we are an adversarial creator of the input that gives bad error, then we can predetermine that we have m bernoulli 50-50 values, that are put at the beginning of each new batch, and the rest are always set 0. Then the $X_i$'s are still iid given the transcript and the proof follows.
Go to the proof of the independence of the inputs given the protocol, and see what happens when the batches are of dynamic size.

We don't know how many batches and what their size, but there will be at most $n$ batches. We want to create randomness apriori (in our seret, for the total error) such that we have randomness for every batch size and current round, which means if we take k more users for the next batch and we are in round t, then this is the error.
Yishay - matrix nxn and row i and column j is the j'th user in the i'th batch (first column is bernoullis and the rest are all zeros). Dynamic error means that dynamically we select for each row how many columns to take.












\begin{theorem}\label{thm:static1shuffler}
For every $\eps$ and $\delta$ such that $\delta<\frac{\min(\eps,1)}{40n}$ and \red{$n^{2/3}c_\eps^{-2/3}\cdot c_{\eps}^2>200^2$}, and any $(\eps,\delta)$-SDP $n$-user single-shuffle algorithm $M$ for private counting under continual observation with static batches. Then there exists an input data set $x \in \{0,1\}^n$ on which $M$ has additive error \red{$\alpha = \Omega(n^{1/3}\cdot c_\eps^{2/3})$} with constant probability.\footnote{Note that for $\eps\ll 1$, $n$ must be at least roughly constant, but for large values of $\eps$, $n$ needs to be very large. This intuitively must hold, since the additive error bound $\alpha$ is sub-constant outside this regime. This makes sense since the weaker the privacy, the weaker the guarantees for large error.}
\end{theorem}
\begin{proof}
Recall that as in the MAB paper, batches came one after the other. 
Let $B_1,\ldots,B_m$ denote the set of predetermined static batches. We split to two cases - one where the largest batch size $\max_{i}\abs{B_i}$ is of size at least \red{$n^{1/3}\cdot c_\eps^{2/3}$ or of size smaller than $c_\eps^{2/3}$.}

For the former case, observe that within the largest batch $B_i$, the error in the count right before the last user can be $\abs{B_i}-1$, since there is no update sent to the server within the batch, and the batch could be all 0's or all 1's. Therefore, on one of those inputs, the probability over $S$ of error at least \red{$\Omega(\max_i\abs{B_i})=\Omega(n^{1/3}\cdot c_\eps^{2/3})$} is at least 1/2.

The rest of the proof focuses on the latter case, where \red{$\max_{i}\abs{B_i}\leq n^{1/3}c_\eps^{2/3}$}. Since wlog we assume that  $\sum_{i=1}^{m}\abs{B_i}=n$ (otherwise we can add new batches that do nothing for the missing users) this means that \red{$m\geq n^{2/3}c_\eps^{-2/3}$}.

Consider a uniformly random input dataset $D = (d_1,\ldots, d_n)$ from the distribution where each $d_i$ is constant 0, except those which are the first of their batch which are sampled i.i.d\ from $Ber(1/2)$. So the sequence looks like $$D\sim (\underbrace{Ber(1/2),0,\ldots,0}_{B_1},\underbrace{Ber(1/2),0,\ldots,0}_{B_2},\ldots,\underbrace{Ber(1/2),0,\ldots,0}_{B_m}).$$
Observe that our sources of randomness is the random vector $D$ and the randomness $S=(S_i)_{i=1}^{m}$ for the shuffle protocols throughout the batches including the encoder randomness and the permutation randomness. Given a concrete $D$ and $S$, denote the transcript of the protocol as sent to the server (the shuffled encoded bits throughout all the batches) by $T = T (D, S)$. 
We now analyze the distribution of the transcript $T$ obtained from $M$ running on a random $D,S$. 
% Observe that a transcript of the algorithm naturally decomposes to the sub-transcript $T_i$ for each static batch $B_i$ during the run of the algorithm, and that a random full transcript of the protocol $T=(T_i)_{i=1}^{m}$ is obtained by concatenating the sub-transcripts $T_i$. Over the distribution $D$, and the run of $M$, each next sub-transcript $t_i$ is deterministically defined based on the previous sub-transcripts $t_{1:i-1}:=(t_1,\ldots,t_{i-1})$ (dictating the used mechanism for batch $i$), randomly selecting a first bit $Ber(1/2)$ (following the distribution of $D$), and using a random source of randomness $S_i$ for the batch.

For $i=1,\ldots,m$, let $i^*$ be the first user of the $i$'th batch, and therefore $d_{i^*}=\sum_{j\in B_i}d_j$ is the true sum of the $i$'th batch.
Fix a batch $i$.
% \red{and condition on an arbitrary prefix of subtranscripts $t_{1:i-1}$, defining the mechanism run in the $i$'th batch.}\blue{TODO: do I need to condition?}
By $(\eps,\delta)$-SDP, since the transcript over the whole algorithm is $(\eps,\delta)$-DP with respect to each input bit, we apply Lemma~\ref{lem:urioverdist} with $M$ as the whole algorithm across all batches, $A$ taken to be the distribution $D$, $Y$ as the total transcript $T$ of the algorithm, $i$ as the current batch we are considering, and $x_1=0$ and $x_2=1$ determine the binary value of $d_{i^*}$. We get that there exists a subset $E_{i}$ of full transcripts of probability $\Pr_{D,S}
[T\in E_i \mid d_{i^*}=1],\Pr_{D,S}[T\in E_i \mid d_{i^*}=0]\geq 1-\frac{2\delta}{\min(\eps,1)}$ such that $\forall t\in E_i$, $\frac{\Pr_{D,S}[T=t \mid d_{i^*}=1]}{\Pr_{D,S}[T=t \mid d_{i^*}=0]}\in [e^{-2\eps},e^{2\eps}]$.
Consider the subset $E=\cap_{i=1}^{m} E_i$ of transcripts $t$ in which for all of the batches $i$ it holds that $\frac{\Pr_{D,S}[T=t \mid d_{i^*}=1]}{\Pr_{D,S}[T=t \mid d_{i^*}=0]}\in [e^{-2\eps},e^{2\eps}]$. By a union bound, it holds that 
% the probability of $E$ is at least $1-O(n\delta/\eps)\geq 0.99$
% , then by Azuma's inequality (Lemma~\ref{lem:azumaCounters}) and since $m\geq n^{2/3}\geq 10$, we get that 
for a random $T$ as defined above, $\Pr_{D,S}[T\in E] \geq 1-\frac{2m\delta}{\min(\eps,1)}\geq 9/10$, where the last step follows by bounds on $\eps$, $\delta$ and $n$ from the Theorem's statement and since $m\leq n$.

Fix a transcript $T=t\in E$. We saw that we receive such a transcript with probability $\geq 0.9$ over $D$ and $S$. Specifically,  for each batch $i$, 

\begin{equation}
    \frac{\Pr_{D,S}[T=t \mid d_{i^*}=1]}{\Pr_{D,S}[T=t \mid d_{i^*}=0]}\in [e^{-2\eps},e^{2\eps}] \label{eq:boundedconditional}
\end{equation}


We claim that:
\begin{enumerate}
    \item The $m$ random variables $\{d_{i^*} \mid T = t\}_{i=1}^{m}$ are independent.
    \item For each batch $i$, $\Pr_{D,S}[d_{i^*} = 1 \mid T=t] \in \left[\frac{1}{e^{2\eps}+1}, \frac{e^{2\eps}}{e^{2\eps}+1}\right]$.
\end{enumerate}
Item 1 follows by Lemma~\ref{lem:independence}, where the parties are the shuffle mechanisms, there are $m$ rounds of communication, and at the $i$'th communication round, only the $i$'th shuffle mechanism communicates a message. This message is a function of the random variable $d_{i^*}$ (the $\{d_{i^*}\}_{i=1}^{m}$'s are initially independent by the definition of $D$), the internal randomness $S_i$, and the outputs of previous shuffle mechanisms which determine the shuffle mechanism that we use. For item 2, observe that for any batch $i$,
\begin{align*}
    \frac{\Pr_{D,S}[d_{i^*}=1 \mid T=t]}{\Pr_{D,S}[d_{i^*}=0 \mid T=t]}&= \frac{\Pr_{D,S}[T=t\mid d_{i^*}=1]\cdot \Pr_{D,S}[d_{i^*}=1]/\Pr_{D,S}[T=t]}{\Pr_{D,S}[ T=t\mid d_{i^*}=0]\cdot \Pr_{D,S}[d_{i^*}=0]/\Pr_{D,S}[T=t]} \\
    &= \frac{\Pr_{D,S}[T=t\mid d_{i^*}=1]\cdot 1/2}{\Pr_{D,S}[ T=t\mid d_{i^*}=0]\cdot 1/2} = \frac{\Pr_{D,S}[T=t\mid d_{i^*}=1]}{\Pr_{D,S}[ T=t\mid d_{i^*}=0]}
    % &=\frac{\Pr_{D,S}[T_{1:i-1}=t_{1:i-1}\mid d_{i^*}=1]}{\Pr_{D,S}[T_{1:i-1}=t_{1:i-1}\mid d_{i^*}=0]}\\
    % &\cdot \frac{\Pr_{D,S}[T_{i}=t_{i}\mid d_{i^*}=1,T_{1:i-1}=t_{1:i-1}]}{\Pr_{D,S}[T_{i}=t_{i}\mid d_{i^*}=0,T_{1:i-1}=t_{1:i-1}]}\\
    % &\cdot \frac{\Pr_{D,S}[T_{i+1:m}=t_{i+1:m}\mid d_{i^*}=1,T_{1:i}=t_{1:i}]}{\Pr_{D,S}[T_{i+1:m}=t_{i+1:m}\mid d_{i^*}=0,T_{1:i}=t_{1:i}]}\\
    % &=\frac{\Pr_{D,S}[T_{i}=t_{i}\mid d_{i^*}=1,T_{1:i-1}=t_{1:i-1}]}{\Pr_{D,S}[T_{i}=t_{i}\mid d_{i^*}=0,T_{1:i-1}=t_{1:i-1}]}\\
    % &=\frac{\Pr_{S_i}[T_{i}=t_{i}\mid d_{i^*}=1,T_{1:i-1}=t_{1:i-1}]}{\Pr_{S_i}[T_{i}=t_{i}\mid d_{i^*}=0,T_{1:i-1}=t_{1:i-1}]}
    \in [e^{-2\eps},e^{2\eps}],
\end{align*}
where the first step follows by Bayes' Rule, the second step follows by the definition of $D$,
% the fourth step follows by the definition of conditional probability for the numerator and denominator separately ($\Pr[A,B,C]=\Pr[A]\cdot \Pr[B\mid A]\cdot \Pr[C\mid A,B]$). The fifth step follows since for the first fraction $d_{i^*}$ does not affect $T_{1:i-1}$, and since for the third fraction while the suffix distribution $T_{i+1:m}$ depends on $d_{i^*}$, the rest of the algorithm is defined based on $T_{1:i}$ which we also condition on. The sixth step follows since $T_i$ is uniquely determined based on $T_{1:i-1}$, $d_{i^*}$ and $S_i$, 
and the last step follows by Equation~(\ref{eq:boundedconditional}). This shows that 
$\Pr_{D,S}[d_{i^*}=1 \mid T=t]\in \left[ \frac{1}{e^{2\eps}+1}, \frac{e^{2\eps}}{e^{2\eps}+1}\right]$.

% Now, observe that the transcript is $(\eps,\delta)$-DP with respect to each bit, so we get that $\Pr_{D,S}[T=t\mid d_{i^*}=1]\leq e^\eps\cdot \Pr_{D,S}[T=t\mid d_{i^*}=0]+\delta$ and $\Pr_{D,S}[T=t\mid d_{i^*}=0]\leq e^\eps\cdot \Pr_{D,S}[T=t\mid d_{i^*}=1]+\delta$. Combined with the equation above, this implies that 
% $\Pr_{D,S}[d_{i^*}=1 \mid T=t]\in \left[\frac{1-\delta}{e^\eps+1},\frac{e^\eps+\delta}{e^\eps+1}\right]\subseteq (1/4,3/4)$,
% since $\eps\in [0,1/2]$ and $\delta \in [0,0.01]$.


Consequently, conditioned on $T = t$, $\sum_{i=1}^{m} d_{i^*}$ is the sum of $m$ independent Bernoulli random variables with bias in $\left[ \frac{1}{e^{2\eps}+1}, \frac{e^{2\eps}}{e^{2\eps}+1}\right]$(variance at least $c_{\eps}^2$) and therefore $\sum_{i=1}^{m} d_{i^*}$ has variance at least $mc_{\eps}^2>200^2$, where the last step follows by the theorem's assumptions on $n$ and $\eps$.

We apply Lemma~\ref{lem:bunetal} to the random variable $(\sum_{j=1}^{n} d_{j}\mid T=t)=(\sum_{i=1}^{m} d_{i^*}\mid T=t)$, 
% we get that there are constants $a,b,c>0$ s.t.\ for all \red{$a\geq \beta\geq2^{-m\cdot \frac{be^{2\eps}}{(e^{2\eps}+1)^2}}$} and every interval $I\in \reals$ of length \red{$\abs{I}\leq c\cdot \sqrt{m\cdot \frac{be^{2\eps}\log (\frac{a}{\beta})}{(e^{2\eps}+1)^2}}$} we have $\Pr_{D,S}[\sum_i d_{i^*}\notin I \mid T=t]\geq \beta$.
% Specifically, for
% 
to the interval $I(t)=M(t) \pm c/2\cdot \sqrt{m\cdot \frac{be^{2\eps}\log (\frac{a}{\beta})}{(e^{2\eps}+1)^2}}$, where $M(t)$ is $M$'s (deterministic) output given the transcript $t$,
% it holds that $\Pr_{D,S}\left[\sum_{j=1}^{n}d_{j} \notin I(t) \mid T=t\right]=\Pr_{D,S}\left[\sum_{i=1}^{m}d_{i^*} \notin I(t) \mid T=t\right]\geq \beta$. We conclude that conditioned on the transcript $t$ and a sufficiently large $n$, if we use 
and the constant $\beta=\min(\frac{a}{4},1/4)\in (2^{-n^{2/3}\cdot \frac{be^{2\eps}}{(e^{2\eps}+1)^2}},a)$, we get that with constant probability over $S$ and $D$ we have error at least $\Tilde{\Omega}(\sqrt{m}\cdot c_\eps)$. Hence, there must exist a fixed input $d\sim D$ for which with constant probability over $S$ we have error at least \red{$\Omega(\sqrt{m}\cdot c_\eps)=\Omega(\sqrt{n^{2/3}c_\eps^{-2/3}}\cdot c_\eps) = \Omega(n^{1/3}\cdot c_\eps^{2/3})$.}

\end{proof}

\begin{theorem}\label{thm:statickshuffler}
For every $\eps$ and $\delta$ such that $\delta<\frac{\min(\eps,1)}{40n}$ and $n^{\frac{2}{2k+1}}\cdot c_{\eps}^{\frac{-2}{2k+1}}c_{\eps}^2>10\cdot 200^2$ \red{THIS BOUND IS BAD}, and any $(\eps,\delta)$-SDP $n$-user $k$-shuffle algorithm $M$ for private counting under continual observation with static batches. Then there exists an input data set $x \in \{0,1\}^n$ on which $M$ has additive error $\alpha = \Omega(Err_{n,k})$ with constant probability.
\end{theorem}
\begin{proof}
% \red{TODO: Set each $T_i$ based on the segment, associate each $T_i$ with the batch $B(i)$ in its center, and claim that by monotonicity since we got DP before wrt the transcript of the batch to $d_{i^*}$, then we also get wrt the whole transcript of the segment. If the segment transcript doesn't even compile since we have batches on each side, find another solution around it.}
We prove the theorem by induction over $k=1,2,\ldots$. The base case $k=1$ is covered in Theorem~\ref{thm:static1shuffler}, \red{however we can instead rely on the base case $k=0$ which is trivial since if there are $k=0$ shufflers, then the error over the either the dataset of all ones or the dataset of all zeros must be at least $n/2$ since their sum difference is $n$ and the outcome of the algorithm is deterministic (since the server is deterministic).}

For the step, let $\eps$, $\delta$ and an $(\eps,\delta)$-SDP $n$-user $k$-shuffle algorithm $M$ for private counting under continual observation with static batches. 

Recall that each shuffler $i=1,\ldots,k$ has its own non-overlapping batches.
We split to two cases: if there exists a batch $B$ of size $\abs{B}\geq Big_{n,k}$, or if all batch $B$ are of size $\abs{B}\leq Big_{n,k}$.

In the former case, if there exists a batch $B$ of size $\abs{B}\geq Big_{n,k}$ of any shuffler, then we focus on that specific batch, and within this batch we have at most $(k-1)$ shufflers running, so by the induction hypothesis within that batch (of size $
abs{B}$ which one can show matches the bounds over $n$ in the Theorem's statement), there exists a sub-input on which we get additive error $\Omega(\abs{B}^{\frac{1}{2k-1}}\cdot c_\eps^{\frac{2k-2}{2k-1}})=\Omega(n^{\frac{2k-1}{(2k+1)(2k-1)}}\cdot c_\eps^{\frac{2}{(2k+1)(2k-1)}}\cdot c_\eps^{\frac{2k-2}{2k-1}})=\Omega(Err_{n,k})$ with constant probability, and extending this sub-input arbitrarily to all the $n$ users, we get the theorem's statement.

For the rest of the proof we assume the latter case, where all batches $B$ are of size $\abs{B}\leq Big_{n,k}$.


Consider a uniformly random input dataset $D = (d_1,\ldots, d_n)$ from the distribution where each $d_i$ is constant 0, except a single $Ber(1/2)$ bit at the middle of each segment of length $10\cdot Big_{n,k}$ bits as below. Specifically the locations of these bits are $(5+10i)\cdot Big_{n,k}$ for $i=1,2,\ldots$ until we reach $n$ users. The sequence looks like $$D\sim (\underbrace{0\ldots 0,Ber(1/2), 0\ldots 0}_{10\cdot n^{\frac{2k-1}{2k+1}}},\ldots,\underbrace{0\ldots 0,Ber(1/2), 0\ldots 0}_{10\cdot n^{\frac{2k-1}{2k+1}}}).$$
 
Observe that our sources of randomness is the random vector $D$ and the shuffle protocols randomness $S=(S_i)_{i=1}^{\#batches}$ for the encoders and the shuffle of all the protocols. Note that the total number of batches is taken over the $k$ shufflers. Also, note that given a concrete $D$ and $S$, since we assume that the server algorithm is deterministic, the random variable denoting the transcript of the protocol as sent to the server (the shuffled encoded bits throughout all the batches) is deterministically defined $T = T (D, S)$.

We now analyze the distribution of the transcript $T$ throughout all batches of all $k$ shufflers obtained from $M$ running on a random $D,S$. We divide the users $d_1,\ldots,d_n$ to segments of $p = 10\cdot Big_{n,k}$ consecutive bits, where we denote by $m=n/p$ the number of such segments. 
Observe that a transcript of the algorithm naturally decomposes to the sub-transcript $T_i$ for each segment $i\in \{1,\ldots,m\}$, where we associate with each segment the set of shuffle encoded inputs of all users of all batches from all the $k$ shufflers that finished during the segment. A random full transcript of the protocol $T=(T_i)_{i=1}^{m}$ is therefore obtained by concatenating the sub-transcripts $T_i$. 
% Over the distribution $D$, and the run of $M$, each next segment $i$'s sub-transcript $t_i$ is deterministically defined based on randomly selecting a first bit $Ber(1/2)$ (following the distribution of $D$), using a random source of randomness $S_j$ for each batch which ends during the segment, which together with the previous sub-transcripts $t_{1:i-1}:=(t_1,\ldots,t_{i-1})$ dictates the used mechanism for each batch associated with the $i$'th segment.


For each $i\in \{1,\ldots,m\}$, let $i^*$ be the index of the $i$'th segment's $Ber(1/2)$ bit, and therefore $d_{i^*}=\sum_{j\in i'th~segment}d_j$ is the true sum of the $i$'th segment. \red{Fix a batch $i$.
% , and condition on an arbitrary prefix of subtranscripts $t_{1:i-1}$
} 
% Observe that $(\eps,\delta)$-SDP implies that the transcript over the set of all batches
% , and specifically the subtranscript associated with the $i$'th segment, 
% is $(\eps,\delta)$-DP with respect to $d_{i^*}$. 
Let $\Sigma_i$ be the concatenation of the randomness $S_j$ of the shufflers $j$ associated with the $i$'th segment. 

By $(\eps,\delta)$-SDP, since the transcript over the whole algorithm is $(\eps,\delta)$-DP with respect to each input bit, we apply Lemma~\ref{lem:urioverdist} with $M$ as the whole algorithm across all batches, $A$ taken to be the distribution $D$, $Y$ as the total transcript $T$ of the algorithm, $i$ as the current segment we are considering, and $x_1=0$ and $x_2=1$ determine the binary value of $d_{i^*}$.


% By Lemma~\ref{lem:uri} with respect to the randomness $\Sigma_i$, we get that there exists a subset of subtranscripts $E_{i}$ of the shufflers related to the $i$'th segment, of probability \red{$\Pr_{\Sigma_i}
% [T_i\in E_i \mid d_{i^*}=1,t_{1:i-1}],\Pr_{\Sigma_i}[T_i\in E_i \mid d_{i^*}=0,t_{1:i-1}]\geq 1-O(\delta/\eps)\geq 0.99$ such that $\forall t_i\in E_i$, $\frac{\Pr_{\Sigma_i}[T_i=t_i \mid d_{i^*}=1,t_{1:i-1}]}{\Pr_{\Sigma_i}[T_i=t_i \mid d_{i^*}=0,t_{1:i-1}]}\in [e^{-2\eps},e^{2\eps}]$}.\footnote{The probability is taken over $\Sigma_i$}

We get that there exists a subset $E_{i}$ of full transcripts of probability $\Pr_{D,S}
[T\in E_i \mid d_{i^*}=1],\Pr_{D,S}[T\in E_i \mid d_{i^*}=0]\geq 1-\frac{2\delta}{\min(\eps,1)}$ such that $\forall t\in E_i$, $\frac{\Pr_{D,S}[T=t \mid d_{i^*}=1]}{\Pr_{D,S}[T=t \mid d_{i^*}=0]}\in [e^{-2\eps},e^{2\eps}]$.
Consider the subset $E=\cap_{i=1}^{m}E_i$ of transcripts $t$ in which for all of the batches $i$ it holds that $\frac{\Pr_{D,S}[T=t \mid d_{i^*}=1]}{\Pr_{D,S}[T=t \mid d_{i^*}=0]}\in [e^{-2\eps},e^{2\eps}]$. By a union bound, it holds that for a random $T$ as defined above, $\Pr_{D,S}[T\in E] \geq 1-\frac{2m\delta}{\min(\eps,1)}\geq 9/10$, where the last step follows by bounds on $\eps$, $\delta$ and $n$ from the Theorem's statement and since $m\leq n$.

% Consider the subset $E$ of transcripts $t=(t_1,\ldots,t_m)$ in which in at least $90\%$ of the segments $i$ it holds that \red{$\frac{\Pr_{\Sigma_i}[T_i=t_i \mid d_{i^*}=1,t_{1:i-1}]}{\Pr_{\Sigma_i}[T_i=t_i \mid d_{i^*}=0,t_{1:i-1}]}\in [e^{-2\eps},e^{2\eps}]$. }
% These events are actually dependent, however since for any $i$ and any prefix of subtranscripts $t_{1:i-1}$, each corresponding a respective assignment of success/failure for each event for the transcripts $t_1,\ldots,t_{i-1}$, it holds that the probability of success is at least $0.99$, then by Azuma’s inequality~\ref{lem:azumaCounters} and since $m\geq 10$, we get that for a random $T=(T_1,\ldots,T_m)$ as defined above, $\Pr_{S}[M(T)\in E]
% % \geq1-\Pr_{S}\left[\abs{\sum_{i=1}^{m}1_{T_i\in E_i}-E[\sum_{i=1}^{m}1_{T_i\in E_i}]}\geq 0.05 m\right]\geq 1-2exp\left(\frac{-(0.05 m)^2}{2m\cdot 0.01}\right)
% \geq 9/10$ . 
% This specifically means that $V(G_{t_i})\leq 0.01$. 
Fix a transcript $T=t\in E$. We saw that we receive such a transcript with probability $\geq 0.9$ over $D$ and $S$. Specifically, 
% there exists a set $J_t$ of indices of segments such that $\abs{J_t}\geq 0.9m$ and $\forall i\in J_t,t_i\in E_i$, and therefore 
for each segment $i$,
\begin{equation}
    \frac{\Pr_{D,S}[T=t \mid d_{i^*}=1]}{\Pr_{D,S}[T=t \mid d_{i^*}=0]}\in [e^{-2\eps},e^{2\eps}].\label{eq:ratio-bounddistar}
\end{equation}

We claim that:
\begin{enumerate}
    \item The $m$ random variables $\{d_{i^*} \mid T = t\}_{i=1}^{m}$ are independent.
    \item For each $i$, $\Pr_{D,S}[d_{i^*} = 1 \mid T = t] \in \left[\frac{1}{e^{2\eps}+1}, \frac{e^{2\eps}}{e^{2\eps}+1} \right]$.
\end{enumerate}
Item 1 follows by Lemma~\ref{lem:independence}, where the parties are the sets of shuffle mechanisms associated with the different segments, there are $m$ rounds of communication, and at the $i$'th communication round, only the $i$'th segment communicates a message. This message is a function of the random variable data $d_{i^*}$ (the $\{d_{i^*}\}_{i=1}^{m}$'s are initially independent by the definition of $D$), the internal randomness $\Sigma_i$, and the outputs of all the previous shuffle mechanisms (from the previous segments) as well as the shuffle randomnesses of shufflers within the segment which determine the shuffle mechanisms that we use during the segment.\footnote{
The parties in this resulting protocol are indeed independent parties since we attribute the communication of all the executed shuffle mechanisms which finished during the $i$'th segment to the $i$'th party, and since the only non-constant bit in the $i$'th segment is $d_{i^*}$, so by the definition of the segment size and maximum batch size, we conclude that no batch can contain the random bits of two consecutive shuffle mechanisms.} For item 2, observe that for any batch $i$ and its middle user $i^*$,
\begin{align}
    \frac{\Pr_{D,S}[d_{i^*}=1 \mid T=t]}{\Pr_{D,S}[d_{i^*}=0 \mid T=t]}&= \frac{\Pr_{D,S}[T=t\mid d_{i^*}=1]\cdot \Pr_{D,S}[d_{i^*}=1]/\Pr_{D,S}[T=t]}{\Pr_{D,S}[ T=t\mid d_{i^*}=0]\cdot \Pr_{D,S}[d_{i^*}=0]/\Pr_{D,S}[T=t]} \\
    &= \frac{\Pr_{D,S}[T=t\mid d_{i^*}=1]\cdot 1/2}{\Pr_{D,S}[ T=t\mid d_{i^*}=0]\cdot 1/2} = \frac{\Pr_{D,S}[T=t\mid d_{i^*}=1]}{\Pr_{D,S}[ T=t\mid d_{i^*}=0]}
    % &=\frac{\Pr_{D,S}[T_{1:i-1}=t_{1:i-1}\mid d_{i^*}=1]}{\Pr_{D,S}[ T_{1:i-1}=t_{1:i-1}\mid d_{i^*}=0]}\\
    % &\cdot \frac{\Pr_{D,S}[T_i=t_i\mid d_{i^*}=1,T_{1:i-1}=t_{1:i-1}]}{\Pr_{D,S}[ T_i=t_i\mid d_{i^*}=0,T_{1:i-1}=t_{1:i-1}]}\\
    % &\cdot \frac{\Pr_{D,S}[T_{i+1:m}=t_{i+1:m}\mid d_{i^*}=1,T_{1:i}=t_{1:i}]}{\Pr_{D,S}[ T_{i+1:m}=t_{i+1:m}\mid d_{i^*}=0,T_{1:i}=t_{1:i}]}\\
    % &=\frac{\Pr_{D,S}[T_i=t_i\mid d_{i^*}=1,T_{1:i-1}=t_{1:i-1}]}{\Pr_{D,S}[ T_i=t_i\mid d_{i^*}=0,T_{1:i-1}=t_{1:i-1}]}\\
    % &=\frac{\Pr_{\Sigma_i}[T_i=t_i\mid d_{i^*}=1,T_{1:i-1}=t_{1:i-1}]}{\Pr_{D,S}[ T_i=t_i\mid d_{i^*}=0,T_{1:i-1}=t_{1:i-1}]}
    \in [e^{-2\eps},e^{2\eps}],
\end{align}
where the first step follows by Bayes' Rule, the second step follows by the definition of $D$,

% the fourth step follows by the definition of conditional probability for the numerator and denominator separately ($\Pr[A,B,C]=\Pr[A]\cdot \Pr[B\mid A]\cdot \Pr[C\mid A,B]$). The fifth step follows since for the first fraction $d_{i^*}$ does not affect $T_{1:i-1}$, and since for the third fraction while the suffix distribution $T_{i+1:m}$ depends on $d_{i^*}$, the rest of the algorithm is defined based on $T_{1:i}$ which we also condition on. The sixth step follows since $T_i$ is uniquely determined based on $T_{1:i-1}$, $d_{i^*}$ and $\Sigma_i$, 
and the last step follows by Equation~\ref{eq:ratio-bounddistar}. This shows that $\Pr_{D,S}[d_{i^*}=1 \mid T=t] \in \left[\frac{1}{e^{2\eps}+1}, \frac{e^{2\eps}}{e^{2\eps}+1} \right]$.

Consequently, conditioned on $T = t$, $\sum_{j=1}^{n} d_{j}=\sum_{i=1}^{m} d_{i^*}$ is the sum of $m$ independent Bernoulli random variables with bias in $\left[\frac{1}{e^{2\eps}+1}, \frac{e^{2\eps}}{e^{2\eps}+1} \right]$ (variance at least $ c_{\eps}^2$) and therefore $\sum_{i=1}^{m} d_{i^*}$ has variance at least $mc_{\eps}^2>200^2$, where the last step follows by the theorem's assumptions on $n$ and $\eps$.

We apply Lemma~\ref{lem:bunetal} to the random variable $(\sum_{j=1}^{n} d_j\mid T=t)=(\sum_{i=1}^{m} d_{i^*}\mid T=t)$, 
% we get that there are constants $a,b,c>0$ s.t.\ for all $a\geq \beta\geq2^{-bm/16}$ and every interval $I\in \reals$ of length $\abs{I}\leq c\cdot \sqrt{bm/16\cdot \log (\frac{a}{\beta})}$ we have $\Pr_{D,S}[\sum_i d_{i^*}\notin I \mid T=t]\geq \beta$.
% Specifically, for 
to the interval $I(t)=M(t) \pm c/2\cdot \sqrt{m\cdot \frac{be^{2\eps}}{(e^{2\eps}+1)^2}\cdot \log (\frac{a}{\beta})}$, where $M(t)$ is $M$'s (deterministic) output given the transcript $t$,
% it holds that $\Pr_{D,S}\left[\sum_{j=1}^{n}d_{j} \notin I(t) \mid T=t\right]=\Pr_{D,S}\left[\sum_{i=1}^{m}d_{i^*} \notin I(t) \mid T=t\right]\geq \beta$. We conclude that conditioned on the transcript $t$ and a sufficiently large $n$, if we use 
and the constant $\beta=\min(\frac{a}{4},1/4)\in (2^{-n^{2/3}\cdot \frac{be^{2\eps}}{(e^{2\eps}+1)^2}},a)$, we get that with constant probability over $S$ and $D$ we have error at least $\Tilde{\Omega}(\sqrt{m}\cdot c_\eps)$. Hence, there must exist a fixed input $d\sim D$ for which with constant probability over $S$ we have error at least $\Omega(\sqrt{m}\cdot c_\eps)=\Omega(\sqrt{n/p}\cdot c_\eps) =\Omega(\sqrt{n/(10\cdot Big_{n,k})}\cdot c_\eps)=\Omega(Err_{n,k})$.\red{Currently this lemma works with constant probability. I can make it work WHP by adding another logn factor to the error.}
\end{proof}
